Quantum-classical convolutional neural networks in radiological image classification

Quantum machine learning is receiving significant attention currently, but its usefulness in comparison to classical machine learning techniques for practical applications remains unclear. However, there are indications that certain quantum machine learning algorithms might result in improved training capabilities with respect to their classical counterparts -- which might be particularly beneficial in situations with little training data available. Such situations naturally arise in medical classification tasks. Within this paper, different hybrid quantum-classical convolutional neural networks (QCCNN) with varying quantum circuit designs and encoding techniques are proposed. They are applied to two- and three-dimensional medical imaging data, e.g. featuring different, potentially malign, lesions in computed tomography scans. The performance of these QCCNNs is already similar to the one of their classical counterparts -- therefore encouraging further studies towards the direction of applying these algorithms within medical imaging tasks.

==> parameters_table.tex <==
\begin{table}[htbp]
\caption{2D convolutional layer parameter count}
\begin{center}
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{}&\multicolumn{3}{|c|}{\textbf{Convolutional layer type}} \\
\cline{2-4} 
\textbf{}& \textbf{\textit{Classical}}& \textbf{\textit{Basic entangling}}& \textbf{\textit{Strongly entangling}} \\
\hline
\multirow{2}{*}{\# parameters}& $2\cdot 2\cdot 4 + 4$& $4 \cdot 1 \cdot 1 $&  $12 \cdot 1 \cdot 1 $\\
& Total: 20 & Total: 4 & Total: 12 \\

\hline
%\multicolumn{4}{1}{Number of trainable parameters in the classical and quantum convolutional layers. Encoding makes no difference. Describe calculation.}

\end{tabular}
}
\label{tab1}
\end{center}

\end{table}



\begin{table}[htbp]
\caption{3D convolutional layer parameter count}
\begin{center}
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{}&\multicolumn{3}{|c|}{\textbf{Convolutional layer type}} \\
\cline{2-4} 
& \multirow{2}{*}{Classical}& \textbf{\textit{Strongly ent.}}& \textbf{\textit{Strongly ent.}} \\
&  & 1 layer & 2 layers \\

\hline
\multirow{2}{*}{\# parameters}& $2\cdot 2\cdot 8 \cdot 64 / 8 + 64 + 128$& $24 \cdot 1 \cdot 8 $&  $24 \cdot 2 \cdot 8 $\\
& Total: 704 & Total: 192 & Total: 386 \\

\hline
%\multicolumn{4}{1}{Number of trainable parameters in the classical and quantum convolutional layers. Encoding makes no difference. Describe calculation.}

\end{tabular}
}
\label{tab2}
\end{center}

\end{table}



\todo{How to make a caption with this template? Title should appear above in capital letters, but what about a more detailed description?}
